NNLO QCD corrections to $pp \to \gamma^* \gamma^*$ in the large $N_F$ limit

We compute the NNLO QCD corrections for the hadroproduction of a pair of off-shell photons in the limit of a large number of quark flavors. We perform a reduction of the two-loop amplitude to master integrals and calculate the latter analytically as a Laurent series in the dimensional regulator using modern integration methods. Real radiation corrections are evaluated numerically with a direct subtraction of infrared limits which we cast in a simple factorized form. The results presented here constitute a gauge invariant part of the full NNLO corrections but are not necessarily dominant. We view this calculation as a step towards a complete computation. Our partial corrections to the total cross-section are about $1\%-3\%$ and vary with the virtuality of the two off-shell photons.

==> masterintegrals.tex <==
% ---------- 2 LOOP ---------- %

\def\sunset#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,28)(92,28)
    \Arc(52,28)(24,0,360)
    \Text(-4,24)[lb]{$p_{34}$}
  \end{picture}
 \end{picture}
}

\def\triangleones#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(28,52)
    \Line(12, 4)(28, 4)   
    \Line(28,52)(76,28)
    \Line(28,4)(76,28)
    \Line(28,52)(28, 4)
    \Line(76,28)(92,28)
    	\Arc(56,28)(37,140,220)
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,24)[lb]{$p_{34}$}
  \end{picture}
 \end{picture}
}

\def\triangletwos#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(28, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(28, 4)
    \Arc(56,28)(37,140,220)
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(-4, 0)[lb]{$p_{24}$}
    	\Text(96,48)[lb]{$p_3$}
  \end{picture}
 \end{picture}
}

\def\Bone#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(92, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(76, 4)
    \Arc[clock](48,28)(37,40,320)
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,48)[lb]{$p_3$}
    	\Text(96, 0)[lb]{$p_4$}
  \end{picture}
 \end{picture}
}

\def\Bonea#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(92, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(76, 4)
    \Arc(56,28)(37,140,220)
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,48)[lb]{$p_3$}
    	\Text(96, 0)[lb]{$p_4$}
  \end{picture}
 \end{picture}
}

\def\Boneb#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(92, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(76, 4)
    \Arc(52,24)(37,50,130)
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,48)[lb]{$p_3$}
    	\Text(96, 0)[lb]{$p_4$}
  \end{picture}
 \end{picture}
}

\def\Btwo#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(92, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(76, 4)
    \Arc[clock](48,28)(37,40,320)
    \Vertex(76,28){3}
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,48)[lb]{$p_3$}
    	\Text(96, 0)[lb]{$p_4$}
  \end{picture}
 \end{picture}
}

\def\Btwoa#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(92, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(76, 4)
    \Arc(56,28)(37,140,220)
    \Vertex(28,28){3}
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,48)[lb]{$p_3$}
    	\Text(96, 0)[lb]{$p_4$}
  \end{picture}
 \end{picture}
}

\def\Btwob#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(92, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(76, 4)
    \Arc(52,24)(37,50,130)
    \Vertex(52,52){3}
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,48)[lb]{$p_3$}
    	\Text(96, 0)[lb]{$p_4$}
  \end{picture}
 \end{picture}
}

% ---------- 1 LOOP ---------- %

\def\bubble#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,28)(28,28)
    \Line(76,28)(92,28)
    \Arc(52,28)(24,180,540)
    \Text(-4,24)[lb]{$p_{34}$}
  \end{picture}
 \end{picture}
}

\def\onelooptriangle#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,28)(28,28)
    \Line(28,28)(76,52)
    \Line(28,28)(76, 4)
    \Line(76,52)(76, 4)
    \Line(76,52)(92,52)
    \Line(76, 4)(92, 4)
    \Text(96,48)[lb]{$p_3$}
    \Text(96, 0)[lb]{$p_4$}
    \Text(-4 ,24)[lb]{$p_{12}$}
  \end{picture}
 \end{picture}
}

\def\oneloopbox#1{
 \begin{picture}(110,60)(0,#1)
  \begin{picture}(110,60)(0,0)
    \SetWidth{1.0}
    %\SetColor{Black}
    \Line(12,52)(92,52)
    \Line(12, 4)(92, 4)   
    \Line(28,52)(28, 4)
    \Line(76,52)(76, 4)
    	\Text(0 ,48)[lb]{$p_1$}
    	\Text(0 , 0)[lb]{$p_2$}
    	\Text(96,48)[lb]{$p_3$}
    	\Text(96, 0)[lb]{$p_4$}
  \end{picture}
 \end{picture}
}
